One Prompt Word is Enough to Boost Adversarial Robustness for Pre-trained Vision-Language Models

Large pre-trained Vision-Language Models (VLMs) like CLIP, despite having remarkable generalization ability, are highly vulnerable to adversarial examples. This work studies the adversarial robustness of VLMs from the novel perspective of the text prompt instead of the extensively studied model weights (frozen in this work). We first show that the effectiveness of both adversarial attack and defense are sensitive to the used text prompt. Inspired by this, we propose a method to improve resilience to adversarial attacks by learning a robust text prompt for VLMs. The proposed method, named Adversarial Prompt Tuning (APT), is effective while being both computationally and data efficient. Extensive experiments are conducted across 15 datasets and 4 data sparsity schemes (from 1-shot to full training data settings) to show APT's superiority over hand-engineered prompts and other state-of-the-art adaption methods. APT demonstrated excellent abilities in terms of the in-distribution performance and the generalization under input distribution shift and across datasets. Surprisingly, by simply adding one learned word to the prompts, APT can significantly boost the accuracy and robustness (epsilon=4/255) over the hand-engineered prompts by +13% and +8.5% on average respectively. The improvement further increases, in our most effective setting, to +26.4% for accuracy and +16.7% for robustness. Code is available at https://github.com/TreeLLi/APT.

==> To_AC.tex <==
Dear AC,

many thanks for coordinating the review of this work.
We would like to raise a special concern about the fairness and credibility of the comment from the reviewer xgZ6. 
Please find below a list of issues raising our concern:

1. 

Although the reviewer xgZ6 claimed xgZ6 is absolutely certain about the evaluation the evaluation  

We are honored to receive valuable feedback from the reviewers and thank you for your assignment. The only concern we have some opinions about is the last reviewer, , who did not understand the paper. 

Almost all the weaknesses xgZ6 mentioned were that he couldn't understand the method. For example, he even couldn't figure out the most basic thing in the field of Adversarial Robustness that the prompt for inference and the prompt for attack are independent to each other. On the other hand, the other two reviewers did not raise any questions about not understanding the method. However, the confidence level the last reviewer xgZ6 gave was five, the highest level, and he thought he understood this method very well.

In conclusion, the reviewer xgZ6 raised the weaknesses which were all about the method understanding and did not understand our method. And the reviewer xgZ6 was very confident while other reviewers can easily understand our method. His evaluation would unfairly judge our paper. 

Kind regards,

Authors

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

To whom it may concern,

We appreciate the insightful feedback provided by the reviewers and express our gratitude for your assessment of our paper. We would like to address a specific concern regarding the comments from the last reviewer, xgZ6.

Our main issue revolves around the fact that Reviewer xgZ6 appears to have difficulty understanding the method in our paper. Many of the weaknesses highlighted by xgZ6 revolve around a misunderstanding of fundamental concepts, such as the independence between the prompt for inference and the prompt for attack in the field of Adversarial Robustness. Remarkably, the other two reviewers did not express any ambiguity regarding the comprehension of our method. It is noteworthy that despite struggling to understand the basics of our approach, Reviewer xgZ6 assigned the highest confidence level, five, which indicates a misunderstanding of our work.

In conclusion, the weaknesses identified by Reviewer xgZ6 pertain solely to a misunderstanding of our method. Given that the other reviewers, who easily comprehended our approach, did not raise similar concerns, we believe that Reviewer xgZ6's evaluation may unfairly impact the overall judgment of our paper.

We kindly request that the committee takes into consideration the discrepancy in understanding and confidence levels among the reviewers in their final assessment of our submission.

Thank you for your time and consideration.

Kind regards,

Authors

